GPT-4V(ision) is a Human-Aligned Evaluator for Text-to-3D Generation

Despite recent advances in text-to-3D generative methods, there is a notable absence of reliable evaluation metrics. Existing metrics usually focus on a single criterion each, such as how well the asset aligned with the input text. These metrics lack the flexibility to generalize to different evaluation criteria and might not align well with human preferences. Conducting user preference studies is an alternative that offers both adaptability and human-aligned results. User studies, however, can be very expensive to scale. This paper presents an automatic, versatile, and human-aligned evaluation metric for text-to-3D generative models. To this end, we first develop a prompt generator using GPT-4V to generate evaluating prompts, which serve as input to compare text-to-3D models. We further design a method instructing GPT-4V to compare two 3D assets according to user-defined criteria. Finally, we use these pairwise comparison results to assign these models Elo ratings. Experimental results suggest our metric strongly align with human preference across different evaluation criteria.

==> figures/i23d_examples/fig.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/diversity_examples/diversity_examples.png}
    \caption{\todo{Image to 3D}}
    \label{fig:diversity}
\end{figure}

==> figures/pairwise/fig.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/pairwise/pairwise.png}
    \caption{\todo{An illustration of how our comparator.}}
    \label{fig:pairwise}
\end{figure}

==> figures/prompt_generator/fig.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/prompt_generator/prompt_generator.pdf}
    \caption{
    \textbf{Prompt generator. }
    L: Existing static prompt libraries invoke a fixed distribution that might overemphasize certain concepts, potentially deviating from an evaluator's intention. R: We propose a prompt generator that can flexibly adapt to different evaluation requirements in terms of complexity and creativity.
    \guandao{People mentioned that this figure doesn't add much information. Can we use Figure 7 here instead?}
    }
    \label{fig:prompt_generator}
\end{figure}

==> figures/radar_chart/fig.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/radar_chart/radar_chart.pdf}
    \caption{\textbf{A holistic evaluation of text-to-3D models.} 
    Our metric allows us to examine these models according to different criteria.
    According to our metrics, the top four models include both optimization-based and feed-forward methods.}
    \label{fig:radar_chart}
\end{figure}

==> sec/1_intro_v0.tex <==
\section{Introduction}
\label{sec:intro}

% \epigraph{The heart of the problem of vision is that the images we see of the world are flat, whereas the world itself is three-dimensional.}{David Marr, \textit{Vision}}

% \epigraph{Sight is the source of knowledge of many things.}{\textit{Aristotle}, \textit{"Metaphysics"}}

\todo{Guandao:change it to focus on text-to-3D.}
% The field of 3D generative models has experienced a Cambrian Explosion in the past years.
The field of 3D generative modeling has witnessed a remarkable expansion in recent years.
This surge can be largely attributed to groundbreaking advancements in neural 3D representations \cite{deepsdf, imnet, nerf}, the availability of large-scale datasets \cite{shapenet, objectverse, objectversexl}, the development of robust generative models \cite{vae, gan, diff-model, score-sde}, and as well as the ability to leverage large foundation pretrained models in text and images~\cite{dreamfusion,etc}.
With these tools, researchers have introduced \todo{numerous} algorithms capable of creating detailed 3D objects from minimal user inputs, such as single images \cite{todo} or textual descriptions \cite{dreamfusion, more}.

% The field of text-to-3D generative methods has experienced a Cambrian Explosion in the past year.
% Such advance is enabled by numerous factor, including the invention of neural 3D representations \cite{deepsdf, imnet, nerf}, the availability of large-scale datasets \cite{shapenet, objectverse, objectversexl}, the emergence of scalable generative models \cite{vae, gan, diff-model, score-sde}, and the ability to leverage large foundation pretrained models in text and images~\cite{dreamfusion,etc}.
% Despite recent advances in 3D generative models, the development of adequate evaluation metrics has not kept pace.

% \todo{(motivate why we need metric)}

Existing metrics tailored for such conditioned 3D generation tasks, such as CLIP Similarity and \todo{others}, often focus on a single evaluation criteria, such as how well the shape aligns with the input text prompt.
As a results, these metrics often lack the flexibility to meet satisfy the broad spectrum of 3D evaluation requirements, such as the quality of 3D shapes. \todo{an examples?}
Furthermore, previous studies have shown that these heuristic-based metrics might not align with human judgment~\cite{he2023t,kirstain2023pick}.
Consequently, many researchers continue to rely on user studies for comprehensive and accurate assessment. 
While well-designed user studies offer adaptability to different evaluation requirements and accuracy in reflecting human judgment, they are also time-consuming and costly. 
% This predicament raises a question: 
This situation raises a question: 
\textit{Can we create automatic metrics that are versatile for various evaluation tasks and align closely with human judgment?}


Creating metrics that meet these criteria is challenging as it demands both an understanding of human intentions and the ability to reason within our three-dimensional physical world.
% Creating metrics that satisfy these criterias is challenging \todo{because it requires both the ability to understand human intention and to conduct common sense reasoning about our three-dimensional physical world}.
 Fortunately, Large Multimodal Models (LMMs) have recently shown promise toward this regard, possessing capabilities for both interpreting user intentions and reasoning about images ~\cite{yang2023dawn}.
% Fortunately, Large Multimodel Models (LMM) have emerged to be powerful tools that process both the ability to understand user intention and the ability to reason about images~\todo{cite-Yangetal2023}.
Similarly to how humans perceive the 3D world through two-dimensional visual information, we hypothesize that LMMs, when adequately trained with extensive data, are capable of performing various 3D model evaluation tasks.
% Just as human are able to perceive the 3D world via \todo{(mention binocular effects?)}two-dimensional visual information, we hypothesize that LMMs, when trained with sufficient scale and data, is capable of conducting different 3D model evaluation tasks.

In this paper, we present a proof-of-concept demonstrating the use of a state-of-the-art Large Multimodal Model, specifically GPT4-Vision (GPT4-V), to develop customizable, accurate, and human-aligned evaluation metrics for 3D generative models. 
Our approach involves designing a framework that effectively prompts GPT4-V to undertake specific 3D evaluation tasks, hinging on several critical design decisions.
\todo{guandao: change it to reflect the method section.}
First, since GPT4-V takes only visual signal yet we need to evaluate 3D shapes, we investigate various ways to create image representations to encode the underlying 3D shapes.
Second, we need to instruct unambiguously GPT4-V how to conduct various 3D evaluation tasks. 
Toward this end, we develop various text prompts for a set of common 3D evaluation tasks, \todo{combining techniques such as visual prompting, chain-of-thoughts, and self-reflection.}
Finally, we need to take GPT4-V's output in the form of natural languages to create a robust quantitative metric.
Ideally, such quantitative measure should be robust toward variance of GPT4-V's response.
To achieve this, we design an ensemble method to gather information from GPT4-V's prompt and create a score for each method \todo{under certain evaluation criteria}.
\todo{(check results)}


Empirically, we showed that the proposed framework achieves the best alignment with human judgment compared to existing automatic metrics.
We also demonstrate that our proposed method is flexible to adapt to different evaluation criteria (Section~\todo{}) and different 3D generation tasks such as single image to 3D (Section~\todo{}).
% Further, we show that our framework is versatile for different evaluation tasks, including both text-to-3d, image-to-3d evaluation, and other application including picking the best 3D generative shapes.
\todo{(check) Finally, we demonstrate that our framework is efficient, capable of producing high quality result by examining model's output with only a few inputs.}

% To summarize, in this paper we provide the proof-of-concept that LMM like GPT4-V can be used to evaluate 3D generative models.
% We propose a framework to create such automatic evaluation metrics that are versatile, accurate, and efficient automatic.
% \todo{We hope that our proposed method is able to guide the development of better 3D geenrative model.}
% We provide initial empirical results.
% Our contributions include:
% \begin{enumerate}
%     \item framework
%     \item data for prompting this 
% \end{enumerate}







% \todo{Prompt selections:
% - lack comprehensive
% - out-of-domain prompt
% - prior works: 
%     - T3Bench
% IDEA: maybe this is orthogonal to contribution of evaluation?
% Contribution: prompt generation prompt "meta-prompt"
%     - Vision provides unique opportunities : prompt generator 
%     - efficiency
%     - finding "differentiating prompt"
% }

% \todo{
% Evaluation dimensions:
% - text-3D-alignment (existing, but we do pretty good)
% - 3D plausibility (physics, common sense, we have advantages)
% --------
% - diversity (new, but emerging and important)
% --------
% - geometry quality (new, emerging)
% - texture quality (new, emerging, might be hard)
% }

% \todo{
% Versatile/customization:
% - image-to-3D and text-to-3D evaluation (Qualitative)
%     - DMV-3D
%     - Shape-E
%     - Point-E
%     - Zero-123
%     - Magic-123
%     - 12345
%     - Wonder3D
%     (Objectverse)
% - evaluation criteria 
% }

==> tables/instance_acc.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \small
  \caption{\textbf{Pair-wise prediction accuracy.}\todo{add scores}}
    \begin{tabular}{l|cccc|c}
          & Alignment & Plausibility & Texture & Geometry & Overall \\
    \midrule
    CLIP  &       &       &       &       &  \\
    Aesthetic &       &       &       &       &  \\
    PickScore &       &       &       &       &  \\
    Human* &       &       &       &       &  \\
    Ours  &       &       &       &       &  \\
    \bottomrule
    \end{tabular}%
  \label{tab:instance_acc}%
\end{table}%

